Is the High-Resolution Coronal Imager Resolving Coronal Strands? Results from AR 12712

Following the success of the first mission, the High-Resolution Coronal Imager (Hi-C) was launched for a third time (Hi-C 2.1) on 29th May 2018 from the White Sands Missile Range, NM, USA. On this occasion, 329 seconds of 17.2 nm data of target active region AR 12712 was captured with a cadence of ~4s, and a plate scale of 0.129''/pixel. Using data captured by Hi-C 2.1 and co-aligned observations from SDO/AIA 17.1 nm we investigate the widths of 49 coronal strands. We search for evidence of substructure within the strands that is not detected by AIA, and further consider whether these strands are fully resolved by Hi-C 2.1. With the aid of Multi-Scale Gaussian Normalization (MGN), strands from a region of low-emission that can only be visualized against the contrast of the darker, underlying moss are studied. A comparison is made between these low-emission strands with those from regions of higher emission within the target active region. It is found that Hi-C 2.1 can resolve individual strands as small as ~202km, though more typical strands widths seen are ~513km. For coronal strands within the region of low-emission, the most likely width is significantly narrower than the high-emission strands at ~388km. This places the low-emission coronal strands beneath the resolving capabilities of SDO/AIA, highlighting the need of a permanent solar observatory with the resolving power of Hi-C.

==> bib_arw.tex <==
@ARTICLE{handy1999,
    author = {{Handy}, B. N. and {Acton}, L. W. and {Kankelborg}, C. C. and 
        {Wolfson}, C. J. and {Akin}, D. J. and {Bruner}, M. E. and {Caravalho}, R. and 
        {Catura}, R. C. and {Chevalier}, R. and {Duncan}, D. W. and 
        {Edwards}, C. G. and {Feinstein}, C. N. and {Freeland}, S. L. and 
        {Friedlaender}, F. M. and {Hoffmann}, C. H. and {Hurlburt}, N. E. and 
        {Jurcevich}, B. K. and {Katz}, N. L. and {Kelly}, G. A. and 
        {Lemen}, J. R. and {Levay}, M. and {Lindgren}, R. W. and {Mathur}, D. P. and 
        {Meyer}, S. B. and {Morrison}, S. J. and {Morrison}, M. D. and 
        {Nightingale}, R. W. and {Pope}, T. P. and {Rehse}, R. A. and 
        {Schrijver}, C. J. and {Shine}, R. A. and {Shing}, L. and {Strong}, K. T. and 
        {Tarbell}, T. D. and {Title}, A. M. and {Torgerson}, D. D. and 
        {Golub}, L. and {Bookbinder}, J. A. and {Caldwell}, D. and {Cheimets}, P. N. and 
        {Davis}, W. N. and {Deluca}, E. E. and {McMullen}, R. A. and 
        {Warren}, H. P. and {Amato}, D. and {Fisher}, R. and {Maldonado}, H. and 
        {Parkinson}, C.},
    title = {The transition region and coronal explorer},
    journal = {\solphys},
    year = 1999,
    month = jul,
    volume = 187,
    pages = {229--260},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{depontieu2014,
   author = {{De Pontieu}, B. and {Title}, A.~M. and {Lemen}, J.~R. and {Kushner}, G.~D. and 
	{Akin}, D.~J. and {Allard}, B. and {Berger}, T. and {Boerner}, P. and 
	{Cheung}, M. and {Chou}, C. and {Drake}, J.~F. and {Duncan}, D.~W. and 
	{Freeland}, S. and {Heyman}, G.~F. and {Hoffman}, C. and {Hurlburt}, N.~E. and 
	{Lindgren}, R.~W. and {Mathur}, D. and {Rehse}, R. and {Sabolish}, D. and 
	{Seguin}, R. and {Schrijver}, C.~J. and {Tarbell}, T.~D. and 
	{W{\"u}lser}, J.-P. and {Wolfson}, C.~J. and {Yanari}, C. and 
	{Mudge}, J. and {Nguyen-Phuc}, N. and {Timmons}, R. and {van Bezooijen}, R. and 
	{Weingrod}, I. and {Brookner}, R. and {Butcher}, G. and {Dougherty}, B. and 
	{Eder}, J. and {Knagenhjelm}, V. and {Larsen}, S. and {Mansir}, D. and 
	{Phan}, L. and {Boyle}, P. and {Cheimets}, P.~N. and {DeLuca}, E.~E. and 
	{Golub}, L. and {Gates}, R. and {Hertz}, E. and {McKillop}, S. and 
	{Park}, S. and {Perry}, T. and {Podgorski}, W.~A. and {Reeves}, K. and 
	{Saar}, S. and {Testa}, P. and {Tian}, H. and {Weber}, M. and 
	{Dunn}, C. and {Eccles}, S. and {Jaeggli}, S.~A. and {Kankelborg}, C.~C. and 
	{Mashburn}, K. and {Pust}, N. and {Springer}, L. and {Carvalho}, R. and 
	{Kleint}, L. and {Marmie}, J. and {Mazmanian}, E. and {Pereira}, T.~M.~D. and 
	{Sawyer}, S. and {Strong}, J. and {Worden}, S.~P. and {Carlsson}, M. and 
	{Hansteen}, V.~H. and {Leenaarts}, J. and {Wiesmann}, M. and 
	{Aloise}, J. and {Chu}, K.-C. and {Bush}, R.~I. and {Scherrer}, P.~H. and 
	{Brekke}, P. and {Martinez-Sykora}, J. and {Lites}, B.~W. and 
	{McIntosh}, S.~W. and {Uitenbroek}, H. and {Okamoto}, T.~J. and 
	{Gummin}, M.~A. and {Auker}, G. and {Jerram}, P. and {Pool}, P. and 
	{Waltham}, N.},
    title = "{The Interface Region Imaging Spectrograph (IRIS)}",
  journal = {\solphys},
archivePrefix = "arXiv",
   eprint = {1401.2491},
 primaryClass = "astro-ph.SR",
 keywords = {Heating, chromospheric, Heating, coronal, Chromosphere, models, Chromosphere, active, Corona, active, Magnetic fields, chromosphere, Instrumentation and data management, Spectrum, ultraviolet},
     year = 2014,
    month = jul,
   volume = 289,
    pages = {2733-2779},
      doi = {10.1007/s11207-014-0485-y},
   adsurl = {http://adsabs.harvard.edu/abs/2014SoPh..289.2733D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
